Robust Communication Between Parties with Nearly Independent Preferences

We study finite-state communication games in which the sender's preference is perturbed by random private idiosyncrasies. Persuasion is generically impossible within the class of statistically independent sender/receiver preferences -- contrary to prior research establishing persuasive equilibria when the sender's preference is precisely transparent. Nevertheless, robust persuasion may occur when the sender's preference is only slightly state-dependent/idiosyncratic. This requires approximating an `acyclic' equilibrium of the transparent preference game, generically implying that this equilibrium is also `connected' -- a generalization of partial-pooling equilibria. It is then necessary and sufficient that the sender's preference satisfy a monotonicity condition relative to the approximated equilibrium. If the sender's preference further satisfies a `semi-local' version of increasing differences, then this analysis extends to sender preferences that rank pure actions (but not mixed actions) according to a state-independent order. We apply these techniques to study (1) how ethical considerations, such as empathy for the receiver, may improve or impede comm

==> 0/Intro.tex <==
In many asymmetric information environments the information in question has little intrinsic importance to the informed party. Consumers care about the quality of a product, but quality has little effect on a salesperson's desire to make a sale; a firm may want to hire quality applicants, but high- and low-quality candidates have similar preferences over offers; the public may care whether a politician is likely to advance their preferred policies, but the politician may only care about re-election. 

In each of these examples, both parties care about the action the uninformed party takes (respectively their purchase, job offer, vote), but their preferences are plausibly independent. We mean this in a statistical sense: the preferences of the informed party are unrelated to what the best action is for the uninformed party.

It is common to model communication in these settings using a state-dependent technology, such as signalling or verifiable disclosure. In the absence of such technologies communication in a one-shot game seems intuitively improbable.

Surprisingly, \cite{LR20} shows that the simple technology of cheap talk --- ie. freely chosen unverifiable messages --- allows for persuasive equilibria for a range of independent utilities. For the finite models that we consider, these equilibria rely on agents randomizing in two important ways. Firstly, senders only send messages that they are indifferent between, to create these indifferences with finite actions, it is typically necessary for the receiver to randomize in equilibrium. Secondly, for the receiver to be willing to randomize, they must form specific posterior beliefs, requiring the sender to randomize between messages in specific state-dependent manners.% meaning that informative communication typically relies on randomizing between messages in a state-dependent manner. Secondly, to create these indifferences with finite actions, it is typically necessary for the receiver to randomize as well. 

However the equilibria obtained strictly rely on the sender's preference being \emph{transparent} --- ie. state-independent and public. In reality, this is a strong assumption. Even if agents' possess state-independent preferences, they are likely to exhibit some degree of idiosyncrasy, even if only minute variations in risk aversion. 

However we find that relaxing the assumption of public preferences makes communication impossible under very weak (topologically generic) assumptions.  
%Within the more general space of independent preferences, which allows for idiosyncrasies, persuasion is impossible outside of a small set\footnote{Small set here can formally be understood as a `shy' set, an infinite dimension analog to measure-0.} of very particular preferences which happens to include the simple case of public preferences. Under mild assumptions, we show that the sender's preference does not lie in this set, rendering communication between parties with independent preferences implausible.
%A prior result from \cite{LR20} describes how communication can arise in equilibrium when the sender's preference is precisely state-independent and public. However, such equilibria --- which we refer to as \emph{candidate equilibria} --- are fragile: if the sender's preference is even slightly idiosyncratic, persuasion is no longer possible in equilibrium. In fact, under mild assumptions, only babbling equilibria exist when the sender's and receiver's preferences are independent. Given that reality is rife with idiosyncrasy, we believe that this suggests the original model is missing a key ingredient in its model of persuasion.
%Note that while previous literature focuses primarily on cheap talk models (ie. with message-independent preferences), our results extend to other state-independent communication technologies such as money-burning models.

In this paper, we seek to re-establish persuasion in finite-state, finite-action models by introducing slight state-dependence to the sender's preference. In our model, the sender's preference $u_S$ is composed of a transparent utility $u$ and an idiosyncratic, state-dependent perturbation $V$:
\begin{equation}\label{eq:intro}
    u_S(a,m\rvert s,\omega)=u(a,m)+\epsilon V(a,m\rvert s,\omega)
\end{equation}
where $a$ is the receiver's action, $m$ is the sender's message\footnote{In cheap talk cases, message dependence may be omitted; we include it for generality as it provides interesting extensions at little conceptual cost.}, $s$ is the state, and $\omega$ is the realized idiosycrasy.

An equilibrium is robust to idiosyncrasy if \emph{for any} $V$, we obtain approximating equilibria as $\epsilon\rightarrow 0$. From our analysis of the state-independent case, we know these informative equilibria do not meet this robustness check. We relax this criteria by allowing the support of $V$ to be constrained to a state-dependent open set $\mathscr{O}$. This open set should be understood as idiosyncrasies being aligned by some state-dependent force --- perhaps ethical considerations, slight material incentives, or even weak technical constraints on the message space.

Upper-hemicontinuity as $\epsilon\rightarrow 0$ ensures that the equilibria of our model will approximate equilibria of the transparent preference model (which we term \emph{candidate equilibria}), in which case we say the candidate equilibrium is $\mathscr{O}$-stable, reflecting the dependence on the open set of idiosyncrasies.% the approximated candidate equilibria.

The main result of this paper is a precise characterization of $\mathscr{O}$-stability. A key element of our analysis is \emph{communication graphs}, these are bipartite graphs that describe the sender's strategy. Their vertices are states and messages, with an edge connecting states with each message sent from that state with positive probability. This structure is a coarsening of equilibrium data, as it omits the probability with which each message is sent, nevertheless it is sufficient to analyze $\mathcal{O}$-stability, as it contains the essential data of which indifferences must be maintained.

The structure of our analysis is inherited from the two types of randomization that are inherent to candidate equilibria. In the first case, the necessity of receiver randomizing significantly constrains the equilibrium posterior beliefs of the receiver, and consequently the equilibrium strategies of the sender. We show that under weak (generic) conditions, this constrains the communication graph to be connected and/or contain a cycle.

Secondly, the constraint of $\mathscr{O}$-stability makes it impossible for cyclic indifferences to be robust to an open set of perturbations. A short proof then concludes that under weak (generic) conditions an equilibrium is $\mathscr{O}$-stable iff its communication graph is acyclic and connected.

This acyclic and connected structure is essential for the next stage of our analysis which identifies precisely the maximal set of modifications $\mathscr{O}$ that makes an equilibrium $\mathscr{O}$-stable. This is precisely the set of perturbations satisfying a condition that we call \emph{graph-cyclic monotonicity} due to its resemblance with Mechanism Design's `cyclic monotonicity'. This term is somewhat unfortunate, as cyclically-monotone perturbations exist iff the communication graph is \emph{acyclic}.

Graph-cyclic monotonicity is implied by a \emph{semi-local increasing differences} condition. This stronger condition often proves simpler to check, and we use it liberally in analyzing example perturbations.

We first apply our techniques to ethical perturbations, relating to empathy and lying aversion. These describe situations where the sender's primary concern is their state-independent material payoff, however they defer to ethical considerations as a `tie-breaking' mechanism. Both empathy and lying aversion stabilize acyclic equilibria in two-state environments, but this does not necessarily generalize to environments with more states.

The stabilizing influence of empathy is tied to whether the receiver and the candidate equilibrium order states in the same way. Specifically, if the receiver's problem satisfies a single crossing condition, providing an order on states and actions, then empathy stabilizes a candidate equilibrium iff lower states recommend lower actions in that candidate equilibrium. We provide a natural 3-state example illustrating how empathy may \emph{inhibit} communication when these conditions are not met: this occurs when persuasion requires the receiver to risk a costly error. The empathetic sender may be unwilling to induce this error, leading to a pareto inferior babbling equilibrium.


%The secondary analysis extends to the setting of what we call \emph{translucent} preferences --- preferences whose ordinal ranking of pure outcomes is public and state-independent, but whose ranking of lotteries may be state-dependent. This poses a generic dilemma between simplicity (ie. acyclicity) and clarity (ie. non-connectedness) in models with translucent preferences.

%In the setting of translucent preferences, we further provide sufficient conditions for a large perturbation to preserve a candidate equilibrium. This condition is satisfied in many of our applications. %and may be of particular interest to 



Lying aversion, on the other hand, is in tension with the nature of candidate equilibria, which generally require obfuscating the state. Lies can be incentivized by a higher material payoff, however care must be taken that this does not interfere with the incentives of senders in other states. This is only possible for simple geometries of communication graphs --- specifically either there is only one state where the sender lies, or only one message is ever a lie.

It is possible to stabilize more candidate equilibria with modifications that are flexible with the truth. Our last example demonstrates this with a modification that allows the sender to make vague statements about the state, stabilizing all acyclic candidate equilibria. We interpret this example as communicating through a low-credibility disclosure technology --- it corresponds to perturbing the transparent preference model towards a model of verifiable disclosure.% We interpret this as a weak disclosure game, where the sender reveals some evidence that the state lies within some subset of the state space. However this evidence may be a false fabrication of the sender --- the only distinction is that false evidence is slightly more costly to produce. This may represent a salesperson 

%In our last section, we turn our attention to a few concrete examples of modifications. We find that when there are only two states, The first is other-regarding preferences. We find if the modification to the sender's preference is antipathic --- that is opposite to the receiver's preference --- no communication can occur. Whereas in a two-state setting, an empathic modification --- ie. slightly aligning their preferences --- will stabilize communication. However, when there are three or more states empathy can interfere with communication. These results further clarify the role of `aligning preferences' in cheap talk communication.

%Lastly, we provide an example of a maximally stabilizing modification, which stabilizes any acyclic candidate equilibrium. We interpret this modification a variation of disclosure games, where the sender communicates by revealing pieces of \emph{easily-falsifiable} information that rule out certain states. This illustrates how the presence of even flimsy evidence greatly expands the possibilities for communication.
%We also consider how purely message based (that is action-independent) modifications can stabilize equilibria. We find that in a `weak' disclosure type game --- where the sender discloses information indicating the state lies within some specific subset of the state-space, but also can cheaply falsify such information --- any acyclic equilibrium can be stabilized. However, if the message space only allows for specific claims about the state, lying aversion only stabilizes a few specific geometries of communication.

%these results can be applied to games that are `close' to our cheap talk game. In particular we consider an application to a disclosure game with a small cost of fabricating evidence, and a communication game where the receiver privately observes a \emph{slightly} informative signal. These technologies can be understood as methods of indirectly nudging the sender, and thus can be treated with our techniques. %We then show how this structure allows the analysis of stable cheap talk equilibria for general preferences. We find that acyclic equilibria exist iff the state-dependent component amounts to \emph{on-path bias} for a specific decomposition of the preference. A consequence is that empathy is always a stabilizing force in two-state environments, but not necessarily if there are more states.
%We also show how this result can be applied to environments where the receiver privately observes an informative signal. The knowledge of the state, and the state-dependent likelihood of it generating various signals indirectly induces a state-dependent preference in the sender over the receiver's beliefs. We apply our techniques to study what conditions on the signal can sustain cheap talk in this environment.


%Lastly, we consider a principal-agent model, where the agent is the sender, and the principal has a weak ability to modify the sender's preference away from state-independence. The principal is then able to foster any acyclic equilibrium from the state-independent case, as long as they have the ability to modify the sender's preference (however weakly) in any direction. We show that the principal can always foster an equilibrium where the sender attains at least their worst pure-state utility. 





